Validating WordNet Meronymy Relations using Adimen-SUMO

In this paper, we report on the practical application of a novel approach for validating the knowledge of WordNet using Adimen-SUMO. In particular, this paper focuses on cross-checking the WordNet meronymy relations against the knowledge encoded in Adimen-SUMO. Our validation approach tests a large set of competency questions (CQs), which are derived (semi)-automatically from the knowledge encoded in WordNet, SUMO and their mapping, by applying efficient first-order logic automated theorem provers. Unfortunately, despite of being created manually, these knowledge resources are not free of errors and discrepancies. In consequence, some of the resulting CQs are not plausible according to the knowledge included in Adimen-SUMO. Thus, first we focus on (semi)-automatically improving the alignment between these knowledge resources, and second, we perform a minimal set of corrections in the ontology. Our aim is to minimize the manual effort required for an extensive validation process. We report on the strategies followed, the changes made, the effort needed and its impact when validating the WordNet meronymy relations using improved versions of the mapping and the ontology. Based on the new results, we discuss the implications of the appropriate corrections and the need of future enhancements.

==> commands.tex <==
\newcommand{\update}[1]{\textcolor{blue}{\uwave{#1}}}
\newcommand{\function}[2]{#1_{/#2}}

% Formulas

\newcommand{\tab}{\hspace{20pt}}
\newcommand{\doubletab}{\tab\tab}
\newcommand{\connective}[1]{\bf #1 \;}
\newcommand{\predicate}[1]{\rm #1}
\newcommand{\constant}[1]{\rm #1}
\newcommand{\variable}[1]{\tt ?#1}
\newcommand{\rowVariable}[1]{\tt @#1}
\newcommand{\true}{\it true}
\newcommand{\false}{\it false}

\newcommand{\TT}[1]{#1}
\newcommand{\FT}[1]{\neg #1}

% Axioms

\newcommand{\textVariable}[1]{{\it{?#1}}}
\newcommand{\textConstant}[1]{{\it{#1}}}
\newcommand{\textFunction}[1]{{\it{#1}}}
\newcommand{\textPredicate}[1]{{\it{#1}}}
\newcommand{\metaConstant}[1]{{\it{\dollar #1}}}
\newcommand{\metaPredicate}[1]{{\dollar #1}}
\newcommand{\dollar}{\$}

% Concepts

\newcommand{\SUMOObjectSymbol}{o}
\newcommand{\SUMOClassSymbol}{c}
%\newcommand{\SUMORelationSymbol}{r}
\newcommand{\SUMOIndividualRelationSymbol}{r}
\newcommand{\SUMOClassOfRelationsSymbol}{R}
\newcommand{\SUMOIndividualAttributeSymbol}{a}
\newcommand{\SUMOClassOfAttributesSymbol}{A}

\newcommand{\SUMOObject}[1]{{\textConstant{#1}$_\SUMOObjectSymbol$}}
\newcommand{\SUMOClass}[1]{{\textConstant{#1}$_\SUMOClassSymbol$}}
%\newcommand{\SUMORelation}[1]{{\textConstant{#1}$_\SUMORelationSymbol$}}
\newcommand{\SUMOIndividualRelation}[1]{{\textConstant{#1}$_\SUMOIndividualRelationSymbol$}}
\newcommand{\HoldsIndividualRelation}[2]{{\textConstant{#1}$^{#2}_{\SUMOIndividualRelationSymbol}$}}
\newcommand{\SUMOClassOfRelations}[1]{{\textConstant{#1}$_\SUMOClassOfRelationsSymbol$}}
\newcommand{\SUMOIndividualAttribute}[1]{{\textConstant{#1}$_\SUMOIndividualAttributeSymbol$}}
\newcommand{\SUMOClassOfAttributes}[1]{{\textConstant{#1}$_\SUMOClassOfAttributesSymbol$}}

\newcommand{\SUMOObjectTikZ}[1]{{\constant{#1}_\SUMOObjectSymbol}}
\newcommand{\SUMOClassTikZ}[1]{{\constant{#1}_\SUMOClassSymbol}}
\newcommand{\SUMOIndividualRelationTikZ}[1]{{\constant{\it #1}_\SUMOIndividualRelationSymbol}}
\newcommand{\SUMOClassOfRelationsTikZ}[1]{{\constant{\it #1}_\SUMOClassofRelationsSymbol}}
\newcommand{\SUMOIndividualAttributeTikZ}[1]{{\constant{#1}_\SUMOIndividualAttributeSymbol}}
\newcommand{\SUMOClassOfAttributesTikZ}[1]{{\constant{#1}_\SUMOClassOfAttributesSymbol}}

% WordNet

\newcommand{\synset}[3]{{\it{#1}$_{#3}^{#2}$}}
\newcommand{\pair}[3]{{\it{#1}(#2,#3)}}

\newcommand{\equivalenceMappingSymbol}{=}
\newcommand{\subsumptionMappingSymbol}{+}
\newcommand{\instanceMappingSymbol}{@}
\newcommand{\negatedEquivalenceMappingSymbol}{\widehat{\equivalenceMappingSymbol}}
\newcommand{\negatedSubsumptionMappingSymbol}{\widehat{\subsumptionMappingSymbol}}

\newcommand{\equivalenceMapping}[1]{{\textConstant{#1}$\equivalenceMappingSymbol$}}
\newcommand{\subsumptionMapping}[1]{{\textConstant{#1}$\subsumptionMappingSymbol$}}
\newcommand{\instanceMapping}[1]{{\textConstant{#1}$\instanceMappingSymbol$}}
\newcommand{\negatedEquivalenceMapping}[1]{{\textConstant{#1}$\negatedEquivalenceMappingSymbol$}}
\newcommand{\negatedSubsumptionMapping}[1]{{\textConstant{#1}$\negatedSubsumptionMappingSymbol$}}

\newcommand{\equivalenceMappingOfConcept}[1]{{#1}$\equivalenceMappingSymbol$}
\newcommand{\subsumptionMappingOfConcept}[1]{{#1}$\subsumptionMappingSymbol$}
\newcommand{\instanceMappingOfConcept}[1]{{#1}$\instanceMappingSymbol$}
\newcommand{\negatedEquivalenceMappingOfConcept}[1]{{#1}$\negatedEquivalenceMappingSymbol$}
\newcommand{\negatedSubsumptionMappingOfConcept}[1]{{#1}$\negatedSubsumptionMappingSymbol$}

\newcommand{\equivalenceMappingRelation}{{\it{equivalence}}}
\newcommand{\subsumptionMappingRelation}{{\it{subsumption}}}
\newcommand{\instanceMappingRelation}{{\it{instance}}}

\newcommand{\synsetTikZ}[3]{{\it{#1}_{#3}^{#2}}}

\newcommand{\equivalenceMappingTikZ}[1]{{{\constant{#1}}\hspace{-4pt}\equivalenceMappingSymbol}}
\newcommand{\subsumptionMappingTikZ}[1]{{{\constant{#1}}\subsumptionMappingSymbol}}
\newcommand{\instanceMappingTikZ}[1]{{{\constant{#1}}\instanceMappingSymbol}}
\newcommand{\negatedEquivalenceMappingTikZ}[1]{{{\constant{#1}}\negatedEquivalenceMappingSymbol}}
\newcommand{\negatedSubsumptionMappingTikZ}[1]{{{\constant{#1}}\negatedSubsumptionMappingSymbol}}

\newcommand{\equivalenceMappingTikZOfConcept}[1]{{#1}\hspace{-4pt}\equivalenceMappingSymbol}
\newcommand{\subsumptionMappingTikZOfConcept}[1]{{#1}\subsumptionMappingSymbol}
\newcommand{\instanceMappingTikZOfConcept}[1]{{#1}\instanceMappingSymbol}
\newcommand{\negatedEquivalenceMappingTikZOfConcept}[1]{{#1}\negatedEquivalenceMappingSymbol}
\newcommand{\negatedSubsumptionMappingTikZOfConcept}[1]{{#1}\negatedSubsumptionMappingSymbol}


% Names

\newcommand{\WORDNET}{{WordNet}}
\newcommand{\SUMO}{SUMO}
\newcommand{\Cyc}{Cyc}
\newcommand{\DOLCE}{DOLCE}
\newcommand{\YAGO}{YAGO}
\newcommand{\TPTPSUMO}{TPTP-SUMO}
\newcommand{\ADIMENSUMO}{Adimen-SUMO}
\newcommand{\adimensumo}{Adimen-SUMO}
\newcommand{\FRAMENET}{FrameNet}
\newcommand{\PREDICATEMATRIX}{Predicate Matrix}
\newcommand{\TCO}{EuroWordNet Top Ontology}
